IPO: Your Language Model is Secretly a Preference Classifier

Reinforcement learning from human feedback (RLHF) has emerged as the primary method for aligning large language models (LLMs) with human preferences. While it enables LLMs to achieve human-level alignment, it often incurs significant computational and financial costs due to its reliance on training external reward models or human-labeled preferences. In this work, we propose Implicit Preference Optimization (IPO), an alternative approach that leverages generative LLMs as preference classifiers, thereby reducing the dependence on external human feedback or reward models to obtain preferences. We conduct a comprehensive evaluation on the preference classification ability of LLMs using RewardBench, assessing models across different sizes, architectures, and training levels to validate our hypothesis. Furthermore, we investigate the self-improvement capabilities of LLMs by generating multiple responses for a given instruction and employing the model itself as a preference classifier for Direct Preference Optimization (DPO)-based training. Our findings demonstrate that models trained through IPO achieve performance comparable to those utilizing state-of-the-art reward models for obtaining preferences.

==> Tables/base_vs_instruct.tex <==
% \begin{table*}[h!]
% \centering
% \begin{tabular}{l|cccc|cccc}
% \hline
% \multirow{}{}{Models} & \multicolumn{4}{c|}{Reward Bench} & \multicolumn{4}{c}{RM-Bench} \\
% \cline{2-9}
%  & Code & Math & Chat & Safety & Chat & Chat Hard & Safety & Reasoning \\
% \hline
% Llama-1B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Llama-1B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% Llama-3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Llama-3B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% Llama-8B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Llama-8B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% Mistral-7B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Mistral-7B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% Qwen-3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Qwen-3B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% Qwen-7B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% Qwen-7B-Inst & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

% \hline
% \end{tabular}
% \caption{Base vs Instruct}
% \label{tab:model_comparison}
% \end{table*}

==> Tables/code.tex <==
\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1.3} % Adjust row spacing
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \hline
        \textbf{Models} & \textbf{go} & \textbf{java} & \textbf{cpp} & \textbf{js} \\
        \hline
        Qwen-Coder-7B-Inst & 0 & 0 & 0 & 0  \\ \hline
        Qwen-Coder-3B-Inst & 0 & 0 & 0 & 0 \\ \hline
        Codegemma-7B & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \caption{Accuracy of coding tasks on Code-Specific models from hep benchmark of RewardBench}
    \label{tab:model_accuracy}
\end{table}


==> Tables/dpo_mistral.tex <==
\begin{table*}[h!]
\centering
\definecolor{apricot}{rgb}{0.95, 0.82, 0.62}
\definecolor{lightgray}{rgb}{0.96, 0.96, 0.96}

\begin{tabular}{l ccccc}
\hline
\rowcolor{apricot} 
\multirow{}{}{\textbf{Models}} & \textbf{BBH} & \textbf{Arc Easy} & \textbf{Alpaca-Eval} & \textbf{MMLU} & \textbf{IFEval} \\ \hline
Mistral-Self & \textit{31.20\%} & \textit{77.00\%} & 69.60\% & \textit{33.00\%} & 29.31\% \\ \hline
\rowcolor{lightgray}Mistral-Ours & \textbf{34.60\%} & \textit{82.20\%} & \textbf{78.20\%} & 37.60\% & \textbf{39.19\%} \\ \hline
Mistral-Reward & 30.20\% & \textbf{85.20\%} & \textit{77.40\%} & \textbf{41.00\%} & \textit{31.69\%} \\ \hline
\end{tabular}
\caption{Comparison of different Mistral model variations across multiple benchmarks. Higher values indicate better performance.}
\label{tab:benchmark_comparison}
\end{table*}


==> Tables/math.tex <==
\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1.3} % Adjust row spacing
    \begin{tabular}{|l| c|}
        \hline
        \textbf{Models} & \textbf{math-prm (\%)} \\
        \hline
        Qwen-Math-7B-Inst & 0 \\ \hline
        Qwen-Math-3B-Inst & 0 \\ \hline
        Llemma-7B & 0 \\ 
        \hline
    \end{tabular}
    \caption{Accuracy of math-prm on maths-Specific models.}
    \label{tab:model_accuracy}
\end{table}
